Non-Coherent and Backscatter Communications: Enabling Ultra-Massive Connectivity in 6G Wireless Networks

With the commencement of the 5G of wireless networks, researchers around the globe have started paying their attention to the imminent challenges that may emerge in the beyond 5G (B5G) era. Various revolutionary technologies and innovative services are offered in 5G networks, which, along with many principal advantages, are anticipated to bring a boom in the number of connected wireless devices and the types of use-cases that may cause the scarcity of network resources. These challenges partly emerged with the advent of massive machine-type communications (mMTC) services, require extensive research innovations to sustain the evolution towards enhanced-mMTC (e-mMTC) with the scalable network cost in 6\textsuperscript{th} generation (6G) wireless networks. Towards delivering the anticipated massive connectivity requirements with optimal energy and spectral efficiency besides low hardware cost, this paper presents an enabling framework for 6G networks, which utilizes two emerging technologies, namely, non-coherent communications and backscatter communications (BsC). Recognizing the coherence between these technologies for their joint potential of delivering e-mMTC services in the B5G era, a comprehensive review of their state-of-the-art is conducted. The joint scope of non-coherent and BsC with other emerging 6G technologies is also identified, where the reviewed technologies include unmanned aerial vehicles (UAVs)-assisted communications, visible light communications (VLC), quantum-assisted communications, reconfigurable large intelligent surfaces (RLIS), non-orthogonal multiple access (NOMA), and machine learning-aided intelligent networks. Subsequently, the scope of these enabling technologies for different device types, service types, and optimization parameters is analyzed...

==> Ver4 LaTeX/acro.tex <==
\begin{acronym}[CA-COOK] 
% Give the longest label here so that the list is nicely aligned

\acro{3GPP}{3\textsuperscript{rd} Generation partnership project}
\acro{3-D}{3-Dimensional}
\acro{5G}{5\textsuperscript{th} Generation}
\acro{6G}{6\textsuperscript{th} Generation}

\acro{AcBsC}{Acoustic backscatter communications}
\acro{ADC}{Analog-to-Digital Converter}
\acro{AI}{Artificial intelligence}
\acro{AMPS}{Advanced mobile phone service}
\acro{AoA}{Angle-of-arrival}
\acro{AP}{Access point}
\acro{APM}{Amplitude-phase modulation}
\acro{APSK}{Amplitude-phase shift keying}
\acro{ASK}{Amplitude shift keying}
\acro{AWGN}{Additive white Gaussian noise}

\acro{B2B}{Backscatter-device-to-backscatter-device}
\acro{B5G}{Beyond 5G}
\acro{BAN}{Body area networks}

\acro{BsC}{Backscatter Communications}

\acro{BS}{Base station}

\acro{BER}{Bit error rate}

\acro{CA-COOK}{Chip average chaotic on-off keying}
\acro{CDMA}{Code division multiple access}
\acro{CoMP}{Coordinated multipoint}
\acro{CSI}{Channel State Information}

\acro{D2D}{Device-to-device}
\acro{DCC}{Direct chaotic communication}
\acro{DF}{Decode-and-forward}
\acro{DFDD}{Decision-Feedback differential detector}
\acro{DSP}{Digital signal processor}
\acro{DPSK}{Differential phase shift keying}


\acro{e-MBB}{Enhanced mobile broadband}

\acro{e-mMTC}{Enhanced massive machine-type communications}

\acro{ESPRIT}{Estimation of signal parameters via rotational invariance techniques}

\acro{FDD}{Frequency division duplex}
\acro{FDMA}{Frequency division multiple access}
\acro{FSK}{Frequency shift keying}

\acro{GaN}{Gallium Nitride}
\acro{GDoF}{Generalized Degrees of Freedom}
\acro{GSM}{Global system for mobile}

\acro{HAP}{High-altitude platform}


\acro{IM}{Index modulation}
\acro{IoT}{Internet-of-things}
\acro{ICT}{Information and communication technologies}

\acro{ITU}{International telecommunication union}

\acro{LAP}{Low-altitude platform}
\acro{LIS}{Large intelligent surfaces}
\acro{LoS}{Line-of-sight}
\acro{LRS}{Large reflective surfaces}

\acro{LTE}{Long-term evolution}

\acro{MAC}{Medium access control}
\acro{MAP}{Maximum a posteriori probability}

\acro{MEC}{Mobile edge computing}
\acro{MFSK}{Multiple FSK}
\acro{MIMO}{Multiple-input multiple-output}
\acro{MIS}{Multiple-input single-output}
\acro{ML}{Machine Learning}
\acro{MLh}{Maximum-likelihood}
\acro{mMTC}{Massive machine-type communications}
\acro{mMIMO}{Massive MIMO}
\acro{mmWave}{Millimeter Wave}

\acro{MAP}{Maximum aposteriori probability}
\acro{MRC}{Maximum ratio combining}
\acro{MS}{Multiple symbol}
\acro{MSMA}{Multiple subcarrier multiple access}
\acro{MSDD}{MS differential detector}
\acro{MSDSD}{MS differential sphere detector}
\acro{MUD}{Multi-user detection}
\acro{MUSIC}{Multiple signal classification}

\acro{NFV}{Network function virtualization}
\acro{nLoS}{non-LoS}
\acro{NOMA}{Non-orthogonal multiple access}




\acro{OAM}{Orbital angular momentum}
\acro{OMA}{Orthogonal multiple access}

\acro{OFDM}{Orthogonal frequency division multiplexing}
\acro{OFDMA}{Orthogonal frequency division multiple access}
\acro{OOK}{On-off keying}

\acro{PAM}{Pulse amplitude modulation}
\acro{PDU}{Protocol data unit}
\acro{PLL}{Phase lock loop}
\acro{PLS}{Physical layer security}

\acro{PeM}{Permutation modulation}
\acro{PSK}{Phase shift keying}

\acro{QAM}{Quadratural amplitude modulation}
\acro{QBsC}{Quantum BsC}
\acro{QC}{Quantum computing}
\acro{QI}{Quantum illumination}
\acro{QoS}{Quality of service}
\acro{QPSK}{Quadrature phase shift keying}
\acro{QSAs}{Quantum search algorithms}

\acro{RF}{Radio frequency}
\acro{RFID}{RF identification}
\acro{RLIS}{Reconfigurable LIS} 
\acro{RMS}{Root mean square}

\acro{SC}{Selection combining}
\acro{SD}{Software-defined}
\acro{SDMA}{Space division multiple access}
\acro{SDN}{SD networks}
\acro{SDP}{Semidefinite programming}
\acro{SER}{Symbol error rate}
\acro{SIC}{Successive interference cancellation}
\acro{SIMO}{Single-input multiple-output}
\acro{SISO}{Single-input single-output}
\acro{SS}{Symbol-by-symbol}
\acro{SWIPT}{Simultaneous wireless information and power transfer}


\acro{SM}{Spatial modulation}

\acro{SNR}{Signal-to-noise ratio}

\acro{SR}{Symbiotic Radio}

\acro{SSK}{Space-shift keying}

\acro{TACD}{Total access communication system}
\acro{T2T}{Tag-to-tag}
\acro{TDMA}{Time division multiple access}
\acro{THz}{Terahertz}
\acro{THID}{THz indentification}
\acro{ToA}{Time-of-arrival}

\acro{UAV}{Unmanned aerial vehicles}
\acro{UDN}{Ultra-dense network}
\acro{UHEE}{Ultra-high energy efficiency}
\acro{UHF}{Ultra high frequency}
\acro{URLLC}{Ultra-reliable low-latency communications}

\acro{VLC}{Visible light communications}
\acro{VLBsC}{Visible light BsC}

\acro{W-CDMA}{Wideband-CDMA}
\acro{WiFi}{Wireless fidelity}
\acro{WSN}{Wireless sensor networks}

\end{acronym}
